Language-guided Semantic Mapping and Mobile Manipulation in Partially Observable Environments

Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.

==> acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/acknowledgements.tex <==
\section{Acknowledgements} \label{sec:acknowledgements}
This work was supported in part by the National Science Foundation under grants IIS-1638072 and IIS-1637813, by the Robotics Consortium of the U.S. Army Research Laboratory under the Collaborative Technology Alliance Program Cooperative Agreement W911NF-10-2-0016, and by ARO grants W911NF-15-1-0402 and W911NF-17-1-0188.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/abstract.tex <==
\begin{abstract}
    Recent advances in data-driven models for grounded language understanding have enabled robots to interpret increasingly complex instructions. Two fundamental limitations of these methods are that most require a full model of the environment to be known a priori, and they attempt to reason over a world representation that is flat and unnecessarily detailed, which limits scalability. Recent semantic mapping methods address partial observability by exploiting language as a sensor to infer a distribution over topological, metric and semantic properties of the environment. However, maintaining a distribution over highly detailed maps that can support grounding of diverse instructions is computationally expensive and hinders real-time human-robot collaboration. We propose a novel framework that learns to adapt perception according to the task in order to maintain compact distributions over semantic maps. Experiments with a mobile manipulator demonstrate more efficient instruction following in a priori unknown environments.
\end{abstract}


==> arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/arxiv/approach.tex <==
% !TEX root = corl-2019.tex
\section{Technical Approach} \label{sec:approach}
%
Many contemporary approaches frame natural language understanding as inference over a learned distribution that associates linguistic elements to their corresponding referents in a symbolic representation of the robot's state and action space. The space of symbols $\bm{\Gamma} = \left\{\gamma_1,\gamma_2 ... \gamma_n\right\}$ includes concepts derived from the robot's environment model, such as objects and locations, and includes the viable robot behaviors, such as navigating to a desired location or manipulating a specific object. The distribution over symbols is conditioned on the parse of the utterance $\bm{\Lambda} = \left\{\lambda_1,\lambda_2 ... \lambda_n\right\}$, and a  model of the world $\Upsilon$ that expresses environment knowledge extracted from sensor measurements $\bm{z}_{1:t}$ using a set of perceptual classifiers $\bm{P} = \left\{p_1,p_2 ... p_n\right\}$. Natural language understanding framed as a symbol grounding problem then follows as maximum a posteriori inference over the power set of referent symbols $\mathcal{P}(\bm{\Gamma})$.
%
\begin{equation}
  \bm{\Gamma^*} = \argmax{\mathcal{P}(\bm{\Gamma})} \; p( \bm{\Gamma}  \vert \bm{\Lambda}, \Upsilon)
  \label{eqn:basic-1}
\end{equation}
%
This approach reasons in the context of a known model of the world $\Upsilon$ that is assumed to express all information necessary to ground the given utterance. This precludes language understanding in unobserved (i.e., novel) or partially observed environments for which the world model is incomplete, thereby making accurate inference \eqref{eqn:basic-1} infeasible. To address this problem, we instead treat symbol grounding as inference conditioned on a latent model of the robot's environment $\overline{\bm{\Upsilon}}$. Specifically, we learn a model that exploits environmental information implicit in an utterance to build a distribution over the topological, metric, and semantic properties of the environment
%
\begin{equation}
 p(\overline{\bm{\Upsilon}}_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}),
 \label{eqn:world-distribution}
\end{equation}
%
where $\bm{\Lambda}_{1:t}$, $\bm{z}_{1:t}$, and $\bm{u}_{1:t}$ denote the history of utterances, sensor observations and odometry, respectively, and $\bm{P}$ is the set of classifiers in the robot's perception pipeline. This allows maintaining a world model distribution that not only embeds the perceived entities from sensor data but also models the unperceived information about the environment expressed in the utterance. This enables symbol grounding in unknown or partially observed environments. As we describe shortly, we maintain this distribution using a Rao-blackwellized particle filter, whereby each particle effectively denotes a hypothesized world model $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$.

Treating the environment model as a latent random variable, we formulate symbol grounding as a problem of inferring a distribution over robot behaviors $\overline{\bm{\beta}}_t$. A behavior $\beta_t$ is a representation of the intended robot actions expressed by the symbols in the inferred groundings $\bm{\Gamma^*}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is inferred in the context of the corresponding world $\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t$ and the instruction $\bm{\Lambda}_t$.
%
The optimal trajectory $\bm{x}_{t}^*$ that the robot should take in the context of a distribution of behaviors then amounts to a planning under uncertainty problem formulated as inference
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{i}_t \in \overline{\bm{\Upsilon}}_t} \underbrace{p(\bm{x}_t \vert \beta_t^{i}, \Upsilon_t^i)}_{\text{path planning}} \times
  \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^i)}_{\text{behavior inference}} \times \underbrace{p( \Upsilon_t^i \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P})}_{\text{semantic mapping}}
  \label{eqn:basic-2}
\end{equation}
%
\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
		ap/.style={rectangle, draw=black, text=white, fill=black!40!orange, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		annotation/.style={rectangle, draw=black, text=white, fill=black!40!green, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		behavior/.style={rectangle, draw=black, text=white, fill=black!40!cyan, line width=0.03cm, minimum size=10mm, text width=2.5cm, align=center},
		basic/.style={rectangle, draw=black, fill=white!60, line width=0.03cm, minimum size=6mm, text width=1.5cm},
		% shorten >=1pt,node distance=5cm,on grid,auto
		on grid, auto,
		scale=0.7, every node/.style={transform shape},
		align=center
		]

		\node[basic]    (human)                             {human};
		\node[basic]    (parser)  [above=0.9in of human]                          {parser};
		\node[inner sep=0,minimum size=0,right=1.0in of parser] (inviz) {};
		\node[annotation]   (nluAnnotation)  [right=1.8 in of parser]               {\textbf{NLU} \\ \textbf{annotation inference}};
		\node[ap]       (nluPercp)  [above=0.9in of nluAnnotation]          {\textbf{NLU} \\ \textbf{perception inference}};
		\node[behavior]    (nluBehavior)     [below=0.9in of nluAnnotation]             {\textbf{NLU} \\ \textbf{behavior inference}};
		\node[ap]           (AP)          [right=2in of nluPercp]                  {adaptive perception};
		\node[annotation]   (semMap)      [right=2in of nluAnnotation]                  {semantic mapping};
		\node[inner sep=0,minimum size=0,below=0.4in of semMap] (inviz2) {};
		\node[behavior]    (policy)      [right=2in of nluBehavior]                  {policy planner};
		\node[basic]        (exec)        [right=1.4in of policy]                  {executive};
		\node[basic]        (robot)       [above=of exec, right=1.4in of semMap]                 {robot};

		\draw [->,line width=1pt] (human.north) -- node [left] {\footnotesize instruction} (parser.south);
		\draw [->,line width=1pt] (inviz.north) |- (nluPercp.west);
		\draw [->,line width=1pt] (inviz.south) |- (nluBehavior.west);
		\draw [->,line width=1pt] (parser.east) -- node [ above, align=center, text width=0.7in, pos=0.4] {\footnotesize parse tree\\ $\bm{\Lambda_t}$} (nluAnnotation.west);

		\draw [->,line width=1pt] (AP.south) -- node [right=-0.2cm, align=center, text width=1in] { \footnotesize compact \\ local world $\Upsilon^*_t$} (semMap.north);
		\draw [->,line width=1pt] (nluPercp.east) -- node [above] {\footnotesize detector \\ \footnotesize symbols $\bm{P}^*_t$} (AP.west);
		\draw [->,line width=1pt] (nluAnnotation.east) -- node [above] {\footnotesize annotation \\ \footnotesize symbols $\bm{\alpha}_t$} (semMap.west);
		\draw [->,line width=1pt] (nluBehavior.east) -- node [above] {\footnotesize distribution over \\ \footnotesize behaviors $\overline{\bm{\beta}}_t$} (policy.west);
		\draw [->,line width=1pt] (semMap.south) -- node [right=-0.3cm,align=center, text width=1in] {\footnotesize distribution over maps $\overline{\bm{\Upsilon}}^{*}_t$} (policy.north);
		\draw [->,line width=1pt] (inviz2.west) -| (nluBehavior.north);

		\draw [->,line width=1pt] (policy.east) -- node [above] {\footnotesize goal $g^*_t$} (exec.west);
		\draw [->,line width=1pt] (exec.north) -- node [right] {\footnotesize commands \\ $\bm{a}_t$} (robot.south);
		\draw [->,line width=1pt] (robot.north) |- node [right, align=center, text width=0.7in, pos=0.25] {\footnotesize observations $\bm{z}_{1:t}, \bm{u}_{1:t}$} (AP.east);

		\end{tikzpicture}
	%
	\caption{The system architecture for language understanding in unknown environments using adaptive perception, semantic mapping, and natural language symbol grounding.  The three language understanding models learned from the corpus of annotated instructions are highlighted in bold.}
	\label{fig:system-architecture}
\end{figure}
%
%
As the robot explores its environment, the distribution over world models is updated by incorporating new detections from the robot's perception pipeline and by incorporating information contained in any instructions that follow. Every time an update is made to the world distribution, the optimal trajectory is recomputed.

The ability to ground diverse natural language instructions is inherently linked to the richness of the robot's representation of the environment. However, building highly detailed models of unstructured environments and performing symbol grounding in their context is computationally expensive and places a runtime bottleneck on the model described by Equation~\ref{eqn:basic-2}. A recent line of research~\cite{patki18a,patki2019a} has shown that perception can be adapted by leveraging language to build task-specific, compact world models for efficient symbol grounding. Figure~\ref{fig:system-architecture} shows the architecture of the proposed model that uses adaptive perception for the task of exploratory mobile manipulation in a priori unknown environments. We leverage adaptive perception online to build compact maps of the environment as the robot explores it. We hypothesize that using adaptive perception will improve the computational efficiency of semantic mapping (Eqn.~\ref{eqn:world-distribution}) and behavior inference (Eqn.~\ref{eqn:basic-1}), and thus improve the runtime language understanding (Eqn.~\ref{eqn:basic-2}). In the following sections, we describe each of the individual learned models of the proposed architecture.
%
\subsection{Adaptive Perception}

In practice, a large fraction of the objects and the corresponding symbols are inconsequential to inferring the meaning of an utterance. In such cases, there exists a compact environment representation that is sufficient to interpret the utterance. A recent line of work~\cite{patki18a,patki2019a} proposes adapting the robot's perception pipeline according to the demands of the language utterance. The goal is to quickly provide minimal task-relevant world models that are sufficiently expressive to permit accurate and fast language grounding. Following ~\cite{patki18a} we learn a Distributed Correspondence Graph (DCG)~\cite{paul2018efficient} based probabilistic model that exploits natural language in order to infer a small, succinct subset of perceptual classifiers $\bm{P}^*_t = f\left( \bm{P}, \bm{\Lambda}_t \right)$ as conditioned on the utterance $\bm{\Lambda}_t$. This allows dynamic adaptation of the robot's perceptual capabilities according to the current task resulting in compact models of the world $\Upsilon^*_t$.
%
\begin{figure}[!tb]
  \centering
  \subfigure[cluttered box]{
    \includegraphics[width=0.32\linewidth]{figures/cluttered_box.jpg}
  }\hfil
  \subfigure[exaustive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ep.png}
  }\hfil
  \subfigure[adaptive perception]{
    \includegraphics[width=0.32\linewidth]{figures/ap.png}
  }
  \caption{A comparison of world models generated by (b) exhaustive and (c) adaptive perception after first observing a cluttered box for the instruction ``pick up the ball inside the box''.}
  \label{fig:ap_ep_comparison}
\end{figure}
%

Previously, adaptive perception has been shown to be effective in building compact models of the world from single observations~\cite{patki18a} or a log of past observations~\cite{patki2019a}. The proposed architecture leverages adaptive perception online in the context of SLAM to build compact maps of the novel environment during exploration.

\subsection{Semantic Mapping with Adaptive Perception}
We model the robot's environment as a semantic graph~\cite{walter13} $\bm{\Upsilon}_t = \{\bm{G}_t,\bm{X}_t,\bm{L}_t\}$. The topology $\bm{G}_t$ is comprised of nodes $n_i$ that represent distinct objects and locations and edges $e_{ij}$ that express spatial relationships between pairs of nodes (e.g., as inferred from language and the robot's motion). The metric map $\bm{X}_t$ associates a pose $x_i$ with each node $n_i$ in the graph in similar fashion to pose graph SLAM~\cite{kaess08}. The layer $\bm{L}_t$ expresses semantic attributes of each node (e.g., the type of each region/object and its colloquial name).

In order to follow instructions in a priori unknown environments, we leverage information about the environment implicit in a given utterance to maintain an informed distribution $\overline{\bm{\Upsilon}}_t$ over possible world models. We learn a DCG-based~\cite{paul2018efficient} probabilistic model that exploits natural language to infer a distribution over the available ``annotations'' $\bm{\alpha}_t$ (of which there may be none). These annotations include the type and relative location of different objects and regions in the environment. As an example, consider the instruction ``get the drill from the box''. DCG inference yields a distribution that assigns a high likelihood to annotations that suggest the existence of one or more objects of type ``box'' and ``drill''. High likelihood is associated with spatial relations that express a drill object as being ``inside'' a box object. The instruction can then be grounded in the context of a distribution of hypothesized worlds that incorporate the inferred annotations.

We maintain this distribution via a Rao-Blackwellized particle filter (RBPF)~\cite{doucet00, hahnel03a}, using a sample-based distribution over topologies, a Gaussian distribution over the metric map, and a Dirichlet over semantic information. We sample changes to the topology (as represented by a collection of particles) according to sensor-based observations and language-based annotations. We then update the resulting distribution over the metric map using an extended information filter. Maintaining a distribution over highly detailed world models and grounding instructions in their context is computationally non-trivial and places a bottleneck on the runtime efficiency of instruction following. We depart from previous work~\cite{hemachandra15} by integrating adaptive perception to maintain a distribution over compact maps $\overline{\bm{\Upsilon}}^*_t$ that afford more efficient behavior inference
%
%
\begin{equation}
  p(\overline{\bm{\Upsilon}}^*_t \vert \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}_t^*).
  \label{eqn:approximate-world-distribution}
\end{equation}
%
%

\subsection{Behavior Inference with Adaptive Perception}

We frame the problem of behavior inference as one of inferring a distribution over grounded behaviors $\overline{\bm{\beta}}_t$ for a given utterance in the context of the distribution over hypothesized worlds $\overline{\bm{\Upsilon}}_t$. When the space of symbols (groundings) $\bm{\Gamma}$ is large, the environment $\Upsilon$ is unstructured, and the free-form utterance $\bm{\Lambda}$ is complex and, making exact inference~\eqref{eqn:basic-1} becomes computationally intractable. Distributed Correspondence Graphs (DCG)~\cite{paul2018efficient} employ an approximate factorization of the grounding distribution in Equation~\ref{eqn:basic-1} that assumes conditional independence across the linguistic and symbolic constituents according to the hierarchical structure of language. DCG frames language understanding as an association problem by introducing the notion of correspondence variables $\phi_{ij} \in \bm{\Phi}$ that associate linguistic elements $\lambda_i \in \bm{\Lambda}$ (e.g., words and phrases) with symbols $\gamma_{ij} \in \bm{\Gamma}$.
In practice, a large fraction of the object and region symbols are irrelevant to inferring the meaning of an utterance. In such cases, there exists a compact environment representation $\Upsilon^{*}$ that is sufficient to interpret the utterance. Reasoning over compact world models reduces the size of the search space, improving the complexity of inference. Following our earlier work~\cite{patki18a,patki2019a}, we use adaptive perception to build these compact world representations. DCG inference then follows as a search for the correspondence variables $\bm{\Phi}^*$ that maximize the following factored distribution. Note that the grounding for a phrase depends on the child phrase groundings as contained in the true correspondence $\bm{\Phi}_{ci}$
%
\begin{equation}
  \bm{\Phi}^* = \argmax{\phi_{ij} \in \bm{\Phi}} \; \prod\limits_{ i = 1 }^{ \lvert \bm{\Lambda} \rvert } \prod\limits_{ j = 1 }^{ \lvert \bm{\Gamma} \rvert } p( \phi_{ij} \vert \gamma_{ij}, \lambda_i, \bm{\Phi}_{ci}, \Upsilon^*).
  \label{eqn:dcg-1}
\end{equation}
%
In a priori unknown environments, our framework performs grounding inference (Eqn.~\ref{eqn:dcg-1}) for each hypothesized world in the distribution. Thus the cost of behavior inference tends to be linear in the number of particles used to maintain the world distribution. Due to the computational advantage of performing inference over compact world models, our framework allows to reason over a larger distribution of possible worlds while being time efficient. Behavior inference finally yields a distribution over behaviors $\overline{\bm{\beta}}_t$. Each behavior $\beta^i_t \in \overline{\bm{\beta}}_t$ is parameterized by a type (navigate, retrieve or pickup) and a goal pose $g^i_t \in \bm{G}_t$.


\subsection{Planning Under Uncertainty}
We hypothesize that leveraging adaptive perception for semantic mapping and behavior inference will improve the runtime of the proposed system (Eqn.~\ref{eqn:proposed_model}) compared to our baseline (Eqn.~\ref{eqn:basic-2}).
%
%
\begin{equation}
  \bm{x}^*_t = \argmax{\bm{x}_t \in \bm{X}_t} \; \sum_{\Upsilon^{*i}_t \in \overline{\bm{\Upsilon}}^{*}_t} \underbrace{p(\bm{x}_t \vert \bm{\beta}^{i}_t, \Upsilon_t^{*i})}_{\text{path planning}} \times
  \underbrace{p( \bm{\beta}^{i}_t \vert \bm{\Lambda}_t, \Upsilon^{*i}_t)}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}}
  \label{eqn:proposed_model}
\end{equation}
%
%
Given a distribution over behaviors, identifying a suitable trajectory $\bm{x}^*_t$ amounts to a planning under uncertainty problem. We solve this problem with a policy that greedily chooses the best behavior $\beta_t^*$ that maximizes the following optimization function
%
%
\begin{equation}
  \beta_t^* = \argmax{\beta_t^i \in \overline{\bm{\beta}}_t} \;  \underbrace{\psi(\beta_t^i)}_{\substack{\text{decaying gaussian} \\ \text{cost function}}} \times \underbrace{p( \beta_t^{i} \vert \bm{\Lambda}_t, \Upsilon_t^{*i} )}_{\substack{\text{behavior inference} \\ \text{with adaptive perception}}} \times \underbrace{p( \Upsilon_t^{*i} \vert  \bm{\Lambda}_{1:t}, \bm{z}_{1:t}, \bm{u}_{1:t}, \bm{P}^*_t)}_{\substack{\text{semantic mapping} \\ \text{with adaptive perception}}},
  \label{eqn:proposed_model_2}
\end{equation}
%
%
where $\psi(\beta_t^i) = e^{ - d(r_t,g^i_t)^{2} / 10 }$ is a decaying Gaussian value function with $d(r_t,g^i_t)$ being the Euclidean distance between the robot and the goal location $g^i_t$ corresponding to the behavior $\beta_t^i$. This allows the robot to favor exploring goals that might be less likely but are closer to the robot. This process is repeated until the robot completes the instructed task.

